SMC4PEP: Stochastic Model Checking of Product Engineering Processes

Product Engineering Processes (PEPs) are used for describing complex product developments in big enterprises such as automotive and avionics industries. The Business Process Model Notation (BPMN) is a widely used language to encode interactions among several participants in such PEPs. In this paper, we present SMC4PEP as a tool to convert graphical representations of a business process using the BPMN standard to an equivalent discrete-time stochastic control process called Markov Decision Process (MDP). To this aim, we first follow the approach described in an earlier investigation to generate a semantically equivalent business process which is more capable of handling the PEP complexity. In particular, the interaction between different levels of abstraction is realized by events rather than direct message flows. Afterwards, SMC4PEP converts the generated process to an MDP model described by the syntax of the probabilistic model checking tool PRISM. As such, SMC4PEP provides a framework for automatic verification and validation of business processes in particular with respect to requirements from legal standards such as Automotive SPICE. Moreover, our experimental results confirm a faster verification routine due to smaller MDP models generated from the alternative event-based BPMN models.

==> Further files apart from main tex/bibtex.tex <==
@inproceedings{DBLP:IG15,
	author = {Association, Information Resources},
	title = {Standard and Standardization: Concepts, Methodologies, Tools and Applications},
	publisher = {USA: IGI Global},
	year = {2015}
}
@phdthesis{Hashemi17,
	author    = {Vahid Hashemi},
	title     = {Decision algorithms for modelling, optimal control and verification
	of probabilistic systems},
	school    = {Saarland University, Saarbr{\"{u}}cken, Germany},
	year      = {2017},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{hashemi2016compositional,
	title={Compositional bisimulation minimization for interval Markov decision processes},
	author={Hashemi, Vahid and Hermanns, Holger and Song, Lei and Subramani, K and Turrini, Andrea and Wojciechowski, Piotr},
	booktitle={Language and Automata Theory and Applications},
	pages={114--126},
	year={2016},
	organization={Springer}
}
@inproceedings{GeblerHT12,
	author="Gebler, Daniel
	and Hashemi, Vahid
	and Turrini, Andrea",
	title="Computing Behavioral Relations for Probabilistic Concurrent Systems",
	booktitle= "ROCKS 2012",
	year="2014",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="117--155",
}
@inproceedings{DBLP:BC14,
	author = {Christiane Brünglinghaus},
	title = {Elektronik und Software beherrschen Innovationen im Auto},
	publisher = {Springer Professional},
	year = {2014}
}

@inproceedings{DBLP:conf/ecsa/HageHM20,
	author    = {Hassan Hage and
	Vahid Hashemi and
	Frank Mantwill},
	title     = {Towards a Systems Engineering Based Automotive Product Engineering
	Process},
	booktitle = {Software Architecture - 14th European Conference},
	series    = {Communications in Computer and Information Science},
	volume    = {1269},
	pages     = {527--541},
	publisher = {Springer},
	year      = {2020}
}
@inproceedings{DBLP:DuranRS18,
	author = {Francisco Duran and Camilo Rocha and Gwen Salaün},
	title = {Stochastic Analysis of BPMN with Time in Rewriting Logic},
	booktitle = {Science of Computer Programming}, 
	pages     = {168, pp. 1-17},
	publisher = {Elsevier},
	year = {2018}
}
@inproceedings{DBLP:LukeH14,
	author = {Luke Hebert},
	title = {Specification, Verification and Optimisation of Business Process},
	publisher = {Technical University of Denmark},
	year = {2014}
}
@book{bhise2017automotive,
	title={Automotive Product Development: A Systems Engineering Implementation},
	author={Bhise, V.D.},
	isbn={9781351645812},
	year={2017},
	publisher={CRC Press}
}
@book{verein2004entwicklungsmethodik,
	title={Entwicklungsmethodik f{\"u}r mechatronische Systeme VDI 2206: Design methodology for mechatronic systems},
	author={Verein Deutscher Ingenieure VDI},
	year={2004},
	publisher={VDI}
}
@book{weber2009automotive,
	title={Automotive Development Processes: Processes for Successful Customer Oriented Vehicle Development},
	author={Weber, J.},
	isbn={9783642012532},
	lccn={2009928427},
	year={2009},
	publisher={Springer Berlin Heidelberg}
}
@MISC{OMG:objectmanagementgroup,
	AUTHOR       = "OMG Object Management Group",
	TITLE        = "Business Process Model and Notation (BPMN)",
	YEAR         = "2014",
	HOWPUBLISHED = "Website",
	URL =      {https://www.omg.org/spec/BPMN};

}
@book{DBLP:journals/fac/HanssonJ94,
	author    = {Hans Hansson and
	Bengt Jonsson},
	title     = {A Logic for Reasoning about Time and Reliability},
	journal   = {Formal Asp. Comput.},
	volume    = {6},
	number    = {5},
	year      = {1994},
	pages     = {512-535},
	ee        = {http://dx.doi.org/10.1007/BF01211866},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}
@book{Aspice,
	title = {Automotive SPICE Process Assessment / Reference Model},
	author = {VDA QMC Working Group 13 / Automotive SIG},
	year = {2017},
	publisher = {Automotive SPICE},
	keywords = {Software}
}

@inproceedings{DaveP11,
	author = {Dave Parker},
	title = {Lecture 14 Model Checking for {MDP}s},
	publisher = {University of Oxford, Department Science},
	year = {2011}
}
@inproceedings{DBLP:conf/formats/AndovaHK03,
	author    = {Suzana Andova and
	Holger Hermanns and
	Joost{-}Pieter Katoen},
	editor    = {Kim Guldstrand Larsen and
	Peter Niebert},
	title     = {Discrete-Time Rewards Model-Checked},
	booktitle = {Formal Modeling and Analysis of Timed Systems: First International
	Workshop, {FORMATS} 2003, Marseille, France, September 6-7, 2003.
	Revised Papers},
	series    = {Lecture Notes in Computer Science},
	volume    = {2791},
	pages     = {88--104},
	publisher = {Springer},
	year      = {2003},
	
}
@InProceedings{CHH+13,
	author={Taolue Chen and Ernst Moritz Hahn and Tingting Han and Marta Kwiatkowska and Hongyang Qu and Lijun Zhang},
	title={Model Repair for {Markov} Decision Processes},
	booktitle={Proc. 7th International Symposium on Theoretical Aspects of Software Engineering (TASE'13)},
	year={2013},
	pages={85--92},
	publisher={IEEE},
}
@book{dajsuren2019automotive,
	title={Automotive Systems and Software Engineering: State of the Art and Future Trends},
	author={Dajsuren, Y. and van den Brand, M.},
	isbn={9783030121570},
	year={2019},
	publisher={Springer International Publishing}
}
@book{bhise2017automotive,
	title={Automotive Product Development: A Systems Engineering Implementation},
	author={Bhise, V.D.},
	isbn={9781351645812},
	year={2017},
	publisher={CRC Press}
}
@inproceedings{Gausemeier2013SEInDerIndustriellenPraxis,
	title={Systems Engineering in der industriellen Praxis},
	author={Jürgen Gausemeier and Roman Dumitrescu and Daniel Steffen and Anja Czaja and Olga Wiederkehr and Christian Tschirner},
	year={2013},
	publisher={Heinz Nixdorf Institut, Frauenhofer Institut, UNITY AG}
}
@inproceedings{Glinz2007,
	author = {Martin Glinz, Samuel Fricker},
	title = {Software Quality Selected Chapter, Chapter 7, Process quality},
	publisher = {University of Zürich, Institut for Informatics},
	year = {2007}
}

@InProceedings{10.1007/3-540-46002-0_5,
	author="Kwiatkowska, Marta
	and Norman, Gethin
	and Parker, David",
	editor="Katoen, Joost-Pieter
	and Stevens, Perdita",
	title="Probabilistic Symbolic Model Checking with PRISM: A Hybrid Approach",
	booktitle="Tools and Algorithms for the Construction and Analysis of Systems",
	year="2002",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="52--66",
	abstract="In this paper we introduce PRISM, a probabilistic model checker, and describe the efficient symbolic techniques we have developed during its implementation. PRISM is a tool for analysing probabilistic systems. It supports three models: discrete-time Markov chains, continuous-time Markov chains and Markov decision processes. Analysis is performed through model checking specifications in the probabilistic temporal logics PCTL and CSL. Motivated by the success of model checkers such as SMV, which use BDDs (binary decision diagrams), we have developed an implementation of PCTL and CSL model checking based on MTBDDs (multi-terminal BDDs) and BDDs. Existing work in this direction has been hindered by the generally poor performance of MTBDD-based numerical computation, which is often substantially slower than explicit methods using sparse matrices. We present a novel hybrid technique which combines aspects of symbolic and explicit approaches to overcome these performance problems. For typical examples, we achieve orders of magnitude speed-up compared to MTBDDs and are able to almost match the speed of sparse matrices whilst maintaining considerable space savings.",
	isbn="978-3-540-46002-2"
}

@inproceedings{krishna:hal-01591665,
	TITLE = {{VBPMN: Automated Verification of BPMN Processes}},
	AUTHOR = {Krishna, Ajay and Poizat, Pascal and Sala{\"u}n, Gwen},
	URL = {https://hal.inria.fr/hal-01591665},
	BOOKTITLE = {{13th International Conference on integrated Formal Methods (iFM 2017)}},
	ADDRESS = {Turin, Italy},
	YEAR = {2017},
	MONTH = Sep,
	KEYWORDS = {business processes ; BPMN ; verification ; evolution ; tool ; process algebra ; LNT ; labelled transition system ; model transformation},
	PDF = {https://hal.inria.fr/hal-01591665/file/main.pdf},
	HAL_ID = {hal-01591665},
	HAL_VERSION = {v1},
}


@article{DBLP:journals/ijseke/Lam10,
	author    = {Vitus S. W. Lam},
	title     = {Formal Analysis of {BPMN} Models: a NuSMV-Based Approach},
	journal   = {Int. J. Softw. Eng. Knowl. Eng.},
	volume    = {20},
	number    = {7},
	pages     = {987--1023},
	year      = {2010},
	url       = {https://doi.org/10.1142/S0218194010005079},
	timestamp = {Wed, 22 Jul 2020 22:06:17 +0200},
	biburl    = {https://dblp.org/rec/journals/ijseke/Lam10.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{doi:10.1080/00207540701199677,
	author = { C.   Ou-Yang  and  Y. D.   Lin },
	title = {{BPMN}-based business process model feasibility analysis: a {P}etri net approach},
	journal = {International Journal of Production Research},
	volume = {46},
	number = {14},
	pages = {3763-3781},
	year  = {2008},
	publisher = {Taylor and Francis},	
	URL = { 
	https://doi.org/10.1080/00207540701199677
	},
	
}

@article{article,
	author = {Mendoza Morales, Luis},
	year = {2014},
	month = {08},
	pages = {3-3},
	title = {Business Process Verification: The Application of Model Checking and Timed Automata},
	volume = {17},
	journal = {CLEI Electronic Journal},
}

@inproceedings{enterprisearchitect,
	TITLE = {{Enterprise Architect 15.2 [Software]}},
	AUTHOR = {Sparx Systems Central Europe},
	URL = {https://www.sparxsystems.de},
	YEAR = {2021},
}

@inproceedings{DBLP:DaclinVV15,
	author = {Nicolas Daclin and Bruno Vallespir and Capurlat Vincent},
	title = {Enabling model checking for collaborative process analysis: from BPMN to ‘Network of Timed Automata’},
	publisher = {Taylor and Francis},
	booktitle = {Enterprise Inforation Systems}, 
	volume = {9},
	pages     = {279--299},
	year = {2015}
}

@Inbook{Valmari1998,
	author={Valmari, Antti},
	editor={Reisig, Wolfgang
	and Rozenberg, Grzegorz},
	title={The state explosion problem},
	bookTitle={Lectures on Petri Nets I: Basic Models: Advances in Petri Nets},
	year={1998},
	publisher={Springer Berlin Heidelberg},
	address={Berlin, Heidelberg},
	pages={429--528},
}

@inproceedings{HahnHWZ10,
	author    = {Ernst Moritz Hahn and
	Holger Hermanns and
	Bj{\"o}rn Wachter and
	Lijun Zhang},
	title     = {PARAM: A Model Checker for Parametric Markov Models},
	booktitle = {CAV},
	year      = {2010},
	pages     = {660-664},
}
@article{DBLP:journals/corr/DehnertJK016,
	author    = {Christian Dehnert and
	Sebastian Junges and
	Joost{-}Pieter Katoen and
	Matthias Volk},
	title     = {The Probabilistic Model Checker Storm (Extended Abstract)},
	journal   = {CoRR},
	volume    = {abs/1610.08713},
	year      = {2016},
	url       = {http://arxiv.org/abs/1610.08713},
	eprinttype = {arXiv},
	eprint    = {1610.08713},
	timestamp = {Mon, 13 Aug 2018 16:48:38 +0200},
	biburl    = {https://dblp.org/rec/journals/corr/DehnertJK016.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{hartmanns2014modest,
	title={The Modest Toolset: An integrated environment for quantitative modelling and verification},
	author={Hartmanns, Arnd and Hermanns, Holger},
	booktitle={International Conference on Tools and Algorithms for the Construction and Analysis of Systems},
	pages={593--598},
	year={2014},
	organization={Springer}
}

@inproceedings{hahn2014iscas,
	title={iscas M c: a web-based probabilistic model checker},
	author={Hahn, Ernst Moritz and Li, Yi and Schewe, Sven and Turrini, Andrea and Zhang, Lijun},
	booktitle={International Symposium on Formal Methods},
	pages={312--317},
	year={2014},
	organization={Springer}
}

@Inproceedings{10.1007/978-3-319-43425-4_4,
	author="Hahn, Ernst Moritz
	and Hashemi, Vahid
	and Hermanns, Holger
	and Turrini, Andrea",
	editor="Agha, Gul
	and Van Houdt, Benny",
	title="Exploiting Robust Optimization for Interval Probabilistic Bisimulation",
	booktitle="Quantitative Evaluation of Systems",
	year="2016",
	publisher="Springer International Publishing",
	address="Cham",
	pages="55--71"
}

==> Further files apart from main tex/commands.tex <==
\iffalse
%\iftrue
\usepackage{todonotes} 
\fi
\newcommand{\mystackrel}[2]{%
	\mathrel{\vbox{\offinterlineskip\ialign{%
				\hfil##\hfil\cr
				$\scriptstyle#1$\cr
				\noalign{\kern.2ex}
				$#2$\cr
}}}}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%\usepackage[plain]{algorithm} %[boxed] = mit Kasten
%\usepackage[noend]{algorithmic}
%\algsetup{indent=2em}
%\renewcommand{\algorithmicthen}{}
%
%\newcommand{\algoTrue}{\ensuremath{\mathbf{true}}}
%\newcommand{\algoFalse}{\ensuremath{\mathbf{false}}}
%
%\iffalse
%\newcommand{\procedure}[1]{\texttt{\scshape#1}}
%\newcommand{\QuotientProc}{\procedure{Quotient}}
%\newcommand{\FindSplitProc}{\procedure{FindSplit}}
%\newcommand{\progHeader}[1]{#1}
%\newcommand{\RefineProc}{\procedure{Refine}}
%\newcommand{\BREAKLOOP}{\STATE{\textbf{break};}}
%\newcommand{\ComputeBisimProc}{\procedure{Bisimulation}}
%\newcommand{\ComputeSimProc}{\procedure{Sim}}
%\newcommand{\SameProc}{\procedure{Same}}
%\newcommand{\ViolateProc}{\procedure{Violate}}
%\newcommand{\MinimalProc}{\procedure{Minimal}}
%\fi


\newboolean{useComments}
\input{use-comments}
\definecolor{dark_purple}{rgb}{0.1, 0.0, 0.4}
\definecolor{dark_green}{rgb}{0.0,0.2,0.5}
\definecolor{dark_red}{rgb}{0.85,0, 0}
\ifthenelse{\boolean{useComments}}{%
	\newcommand{\ms}[1]{\todo[inline,color=white!40,bordercolor=white]{\textcolor{teal!70!black!80}{\textbf{Manos:}\textmd{\;#1}}}} 
	\newcommand{\vh}[1]{\todo[inline,color=white!40,bordercolor=white]{\textcolor{purple!70!black!80}{\textbf{Vahid:}\textmd{\;#1}}}}  
	\newcommand{\hh}[1]{\todo[inline,color=white!40,bordercolor=white]{\textcolor{blue!70!black!80}{\textbf{Hassan:}\textmd{\;#1}}}} 
	%        
}{%
	\newcommand{\ms}[1]{}
	\newcommand{\hh}[1]{}
	\newcommand{\vh}[1]{}

}



\newcommand{\SequenceOfFlowsProc}{\procedure{Smf}}
\newcommand{\SequenceOfFlowsInitProc}{\procedure{Smf}_{\mathit{init}}}
%\def\sat{\mathit{Sat}}

\newcommand{\StepCondition}{\procedure{StepCondition}}

\newcommand{\partitioningord}{\relord[R]}
\newcommand{\partitioning}{\rel[W]}

\newcommand{\classToSplit}{{\mathcal C}}
\newcommand{\splitAction}{a}
\newcommand{\splitDistribution}{\gd}

\newcommand{\listener}[1]{\mathit{Listener}(#1)}
\newcommand{\match}{\mathit{match}}
%\usepackage[plain]{algorithm} %[boxed] = mit Kasten
%\usepackage[noend]{algorithmic}
%\algsetup{indent=2em}
%\renewcommand{\algorithmicthen}{}
\newcommand{\distrib}[1]{\Disc{#1}}
\def\prob{\textnormal{Pr}}
\usepackage{bigstrut}
\usepackage{paralist}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{comment}
% \usepackage{caption,subcaption}
%\usepackage{cite}
%\usepackage{clrscode}
%\usepackage{pictexwd}
\usepackage{graphicx}
\usepackage{caption}
%\usepackage{subcaption}
\usepackage{ifthen}
\usepackage{paralist}
%\usepackage{pst-all}
\usepackage{pgf}
% \usepackage{tikz}
\usetikzlibrary{automata,arrows,intersections,positioning,calc,shapes}
%\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{etoolbox}

\newcommand{\algc}[1]{{\textsf{\scriptsize //{}#1}}}
\newcommand{\act}{a}
\newcommand{\acttwo}{b}


\newcommand{\dis}{\sd}
\newcommand{\distwo}{\nu}
\newcommand{\rew}{\mathrm{r}}
\newcommand{\stateRew}{{\rew_{\textit{state}}}}
\newcommand{\actionRew}{{\rew_{\textit{action}}}}
\newcommand{\un}{{(\forall)}}
\newcommand{\ex}{{(\exists)}}
\newcommand{\controlSyn}{{(\exists\sch\forall)}}
\newcommand{\paramSyn}{{(\exists\env\forall)}}
\newcommand{\synthesis}{{(\exists\forall)}}
\newcommand{\functioneval}[2]{#1(#2)}
\newcommand{\pat}{\omega}
\newcommand{\sigmaalgebra}{\mathcal{B}}
\newcommand{\convexComb}[1]{\mathrm{CH}(#1)}
\newcommand{\convexhull}[1]{\convexComb{#1}}

\newcommand{\lifting}[1]{\mathrel{\mathcal{L}(#1)}}

\newcommand{\transition}[2]{{#1 \longrightarrow #2}}
\newcommand{\transitionAction}[3]{{#1 \mystackrel{#2}{\longrightarrow} #3}}
\newcommand{\tra}[1]{{}\mathchoice%
	{\stackrel{#1}{\longrightarrow}}
	% vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
	{\mathop {\smash\longrightarrow}\limits^{\vrule width 0pt height 0pt depth 4pt\smash{#1}}}
	{\stackrel{#1}{\longrightarrow}}
	{\stackrel{#1}{\longrightarrow}}
	{}}

\newcommand{\eqclass}{\mathcal{C}}


\newcommand{\mixedActions}[1]{\mathrm{\distrib{\actionSet_{#1}}}}

%\newcommand{\concreteTransitions}[1]{\mathrm{Transitions(#1)}}
%\newtheorem{result}{Result}
%\newcommand{\bigO}[1]{\mathcal{O}(#1)}

% Andrea: I do not like ordinary epsilon/phi symbol
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\phi}{\varphi}

% Number sets
\newcommand{\reals}{\mathbb{R}}
\newcommand{\posreals}{\reals_{\geq 0}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\naturals}{\mathbb{N}}

\newcommand{\setcond}[2]{\lbrace\, #1 \mid #2 \,\rbrace}
\newcommand{\setnocond}[1]{\{#1\}}

\newcommand{\powerSet}[1]{2^{#1}}

\newcommand{\size}[1]{\left\lvert#1\right\rvert}

\newcommand{\norm}[2][2]{\left\|#2\right\|_{#1}}

% Least common multiple
%\DeclareMathOperator{\lcm}{lcm}

% Generic probability distributions
\newcommand{\sd}{\mu} % states distribution
\newcommand{\gd}{\rho} % generic distribution
\newcommand{\dirac}[1]{\delta_{#1}}

% for generic argument of functions, as f(.)
\newcommand{\functionDot}{\,\cdot\,}

% Sets relative to probability distributions
\newcommand{\Disc}[1]{\Delta(#1)}
\newcommand{\SubDisc}[1]{\mathrm{SubDisc}(#1)}
\newcommand{\Supp}[1]{\mathrm{Supp}(#1)}



\newcommand{\parComp}{\parallel}

% Automata and components
\newcommand{\aut}[1][A]{\mathcal{#1}}
%\newcommand{\mdp}[1][M]{\aut[#1]}
\newcommand{\imdp}[1][M]{\aut[#1]}
\renewcommand{\vec}[1]{{\mathbf #1}}
\newcommand{\stateSet}{S}
\newcommand{\actionSet}{\mathcal{A}}
\newcommand{\stateActionSet}[1]{\actionSet(#1)}
\newcommand{\startState}[1][s]{\bar{#1}}
\newcommand{\intTransitionProbability}{\mathit{I}}

\newcommand{\APSet}{\mathtt{AP}}
\newcommand{\APLabelling}{L}


\newcommand{\interval}[2]{[#1,#2]}
\newcommand{\intervalSet}{\mathbb{I}}

\newcommand{\paths}{\mathit{Paths}}
\newcommand{\pathsfin}{\paths^{*}}
\newcommand{\pathsinf}{\paths^{\omega}}

% Bisimulation symbols
\newcommand{\bisim}{\sim}

\newcommand{\fine}{\mathit{AARC}}



% LP problems
\newcommand{\dotteddiamond}{\kern-1pt\setbox0=\vbox{\hbox{$\diamond$}}{\ooalign{\hfil\box0\hfil\cr\hfil$\mkern-0.5mu \cdot$\hfil\crcr}}\kern-1pt}
\newcommand{\NetworkTBetaRel}[3]{G(#1,#3)}
\newcommand{\LPproblemTBetaMuRel}[3][\relord]{\mathit{LP}(#2,#3,#1)}%{\transition{#2}{\dotteddiamond\liftrel[#1]#3}}}

% Subsets of transitions
\newcommand{\transitionsWithLabel}[1]{\mathord{\mystackrel{#1}{\transitionRelation}}}
\newcommand{\transitionsFromState}[1]{\mathord{\strongTransition{#1}{}{}}}



% Internal action
\newcommand{\hidden}{\tau}
\newcommand{\node}{\mathcal{V}}
%\newcommand{\arc}{\mathcal{E}}
\newcommand{\subArc}{\mathcal{\bar{E}}}
\newcommand{\tran}{\mathcal{T}}


% Generic transition
\newcommand{\tr}{\mathit{tr}}
\newcommand{\source}[1]{\mathit{src}(#1)}
\newcommand{\action}[1]{\mathit{act}(#1)}
\newcommand{\target}[1]{\mathit{trg}(#1)}


\newcommand{\reach}[1]{\mathit{reach}(#1)}
\newcommand{\pre}[1]{\mathit{pre}(#1)}
\newcommand{\post}[1]{\mathit{post}(#1)}
\newcommand{\postbot}[1]{\boted{\mathit{post}}(#1)}

% Sets and operators on execution fragments
\newcommand{\prefix}{\leqslant}
\newcommand{\length}[1]{\lvert #1 \rvert}
\newcommand{\cone}[1]{C_{#1}}
\newcommand{\trace}[1]{\mathit{trace}(#1)}
\newcommand{\last}[1]{\mathit{last}(#1)}
\newcommand{\first}[1]{\mathit{first}(#1)}
\newcommand{\emptytrace}{\epsilon}
\newcommand{\fragRestriction}[2]{#1{\downharpoonright}#2}

% Transitions depicted as arrows
\newcommand{\genericTransition}[4]{{#1 \mystackrel{#2}{\longrightarrow}_{#4} #3}}
\newcommand{\combined}{\mathrm{C}}
\newcommand{\strongTransition}[3]{{#1 \mystackrel{#2}{\longrightarrow} #3}}
\newcommand{\strongCombinedTransition}[3]{{#1 \mystackrel{#2}{\longrightarrow}_{\combined} #3}}
\newcommand{\weakTransition}[3]{{#1 \mystackrel{#2}{\Longrightarrow} #3}}
\newcommand{\weakCombinedTransition}[3]{{#1 \mystackrel{#2}{\Longrightarrow}_{\combined} #3}}
\newcommand{\hyperStrongTransition}[3]{{#1 \mystackrel{#2}{\longrightarrow} #3}}
\newcommand{\hyperStrongCombinedTransition}[3]{{#1 \mystackrel{#2}{\longrightarrow}_{\combined} #3}}

\newcommand{\hyperWeakTransition}[3]{{#1 \mystackrel{#2}{\Longrightarrow} #3}}
\newcommand{\hyperWeakCombinedTransition}[3]{{#1 \mystackrel{#2}{\Longrightarrow}_{\combined} #3}}

% Relations and lifting
\newcommand{\relsymbol}{\mathcal{R}}
%\newcommand{\relord}[1][\relsymbol]{\mathcal{#1}}
\newcommand{\relord}[1][\relsymbol]{#1}
\newcommand{\rel}[1][\relsymbol]{\mathrel{\relord[#1]}}
\newcommand{\idrelsymbol}{I}
\newcommand{\idrelord}[1][\idrelsymbol]{\relord[#1]}
\newcommand{\idrel}[1][\idrelsymbol]{\rel[#1]}
\newcommand{\wbrelsymbol}{W}
\newcommand{\wbrelord}[1][\wbrelsymbol]{\relord[#1]}
\newcommand{\wbrel}[1][\wbrelsymbol]{\rel[#1]}
\newcommand{\liftrel}[1][\relord]{\mathrel{\liftrelord[#1]}}
\newcommand{\liftrelord}[1][\relord]{\mathord{\mathcal{L}(#1)}}
\newcommand{\liftreleps}[1][\relord]{\mathrel{\liftrelepsord[#1]}}
\newcommand{\liftrelepsord}[1][\relord]{\mathrel{\mathcal{L}^\epsilon(#1)}}

\newcommand{\borderTerm}{border}
\newcommand{\borderStateSetOrd}[1][\relord]{\mathcal{B}(#1)}
\newcommand{\borderStateSet}[1][\relord]{\borderStateSetOrd[#1]}
\newcommand{\tool}{\acronym{SMC4PEP}}
\newcommand{\mdp}{\acronym{MDP}}
\newcommand{\pb}{\acronym{pBPMN}}
\newcommand{\eb}{\acronym{eBPMN}}
% Equivalence classes

\newcommand{\relclass}[2]{[#1]_{#2}}
\newcommand{\relimage}[2]{#2(#1)}
\newcommand{\quotienting}[2]{#1/#2}
\newcommand{\partitionset}[2][\relord]{\quotienting{#2}{#1}}

% Generic bisimulation
\newcommand{\genericBisim}{\asymp}
\newcommand{\genericBisimord}{\mathord{\genericBisim}}

% Strong bisimulation
\newcommand{\strongBisim}{\sim}
\newcommand{\strongProbBisim}{\strongBisim_{p}}
\newcommand{\strongBisimApprox}{\strongBisim_{\epsilon}}
\newcommand{\strongBisimord}{\mathord{\strongBisim}}
\newcommand{\strongProbBisimord}{\mathord{\relord[R]}}
\newcommand{\strongBisimApproxord}{\mathord{\strongBisimApprox}}

% Weak bisimulation
\newcommand{\weakBisim}{\approx}
\newcommand{\weakProbBisim}{\weakBisim_{p}}
\newcommand{\weakBisimApprox}{\weakBisim_{\epsilon}}
\newcommand{\weakBisimord}{\mathord{\weakBisim}}
\newcommand{\weakProbBisimord}{\mathord{\weakProbBisim}}
\newcommand{\weakBisimApproxord}{\mathord{\weakBisimApprox}}

% Generic simulation
\newcommand{\genericSim}{\preccurlyeq}
\newcommand{\genericSimord}{\mathord{\genericSim}}

% Strong simulation
\newcommand{\strongSim}{\lesssim}
\newcommand{\strongProbSim}{\strongSim_{p}}
\newcommand{\strongSimApprox}{\strongSim_{\epsilon}}
\newcommand{\strongSimord}{\mathord{\strongSim}}
\newcommand{\strongProbSimord}{\mathord{\strongProbSim}}
\newcommand{\strongSimApproxord}{\mathord{\strongSimApprox}}

% Weak simulation
\newcommand{\weakSim}{\lessapprox}
\newcommand{\weakProbSim}{\weakSim_{p}}
\newcommand{\weakSimApprox}{\weakSim_{\epsilon}}
\newcommand{\weakSimord}{\mathord{\weakSim}}
\newcommand{\weakProbSimord}{\mathord{\weakProbSim}}
\newcommand{\weakSimApproxord}{\mathord{\weakSimApprox}}

% Network related commands
\newcommand{\incomingflow}{\vec{f}}
\newcommand{\netsource}{\mathord{\vartriangle}}
\newcommand{\netsink}{\mathord{\blacktriangledown}}
\newcommand{\network}[1][N]{\mathcal{#1}}
\newcommand{\capacity}{c}


% Acronyms
\newcommand{\acronym}[1]{\ensuremath{\textnormal{#1}}}
\newcommand{\MDP}{\acronym{MDP}}
\newcommand{\IMDP}{\acronym{IMDP}}
\newcommand{\LP}{\acronym{LP}}

\newcommand{\always}{\pmb{\square}}


\newcommand{\J}{\Join}

\newcommand{\nxt}{{\text{\sf X}}}
\newcommand{\unt}{{\text{\sf U}}}
\newcommand{\pctlP}{{\text{\sf P}}}
\newcommand{\true}{\textit{true}}

\newcommand{\hpoly}{{$\mathcal{H}$}-polytope}
%%%%%%%%%%%%%%%%%%%%%

% Uncertain IMDP commands

\newcommand{\cyl}[1]{\mathit{Cyl}_{#1}}   
%
\newcommand{\Sch}{\Sigma}
\newcommand{\Nature}{\mathfrak{N}}
\newcommand{\nature}{\nu}
\newcommand{\sched}{\sigma}

\newcommand{\uncertain}{\mathcal{P}}
\newcommand{\uncertainty}[2]{\uncertain^{#1,#2}}
\newcommand{\paruncertainty}[3]{\uncertain^{#1,#2}_{#3}}
\newcommand{\parcombuncertainty}[2]{\uncertain^{#1}_{#2}}

\newcommand{\pth}{\mathit{Paths}}
\newcommand{\fpth}{\mathit{Paths}_{\mathit{fin}}}
\newcommand{\infpth}{\mathit{Paths}_{\mathit{inf}}}
\newcommand{\ifpth}[1]{\mathit{Paths}_{#1}}   
%

\newcommand{\Sched}{\emph{Scheduler}}
\newcommand{\Envir}{\emph{Nature}}

\newcommand{\envir}{\emph{nature}}
\newcommand{\Env}{\Pi}
\newcommand{\env}{\pi}
\newcommand{\sch}{\sigma}
\newcommand{\probability}{\textit{Prob}}
\newcommand{\ssch}{\sch\in\Sch}
\newcommand{\senv}[1]{\pi_{#1}\in\Env}
\newcommand{\fixedUncertainty}[2]{{\mu}_{#1}^{#2}}
\newcommand{\elementFixedUncertainty}[3]{{\mu}_{#1}^{#3}[#2]}
\newcommand{\validUncertainty}[2]{\mathcal{F}_{#1}^{#2}}
\newcommand{\adv}{\mathit{Adv}}
\newcommand{\advdt}{\mathit{Adv}_\mathit{dt}}
\newcommand{\advha}{\mathit{Adv}_\mathit{ha}}
\newcommand{\advst}{\mathit{Adv}_\mathit{st}}
\newcommand{\advhd}{\mathit{Adv}_\mathit{hd}}
\newcommand{\advsi}{\mathit{Adv}_\mathit{si}}
%\newcommand{\last}{\mathit{last}}
%\newcommand{\length}{\mathit{length}}

\newcommand{\ind}{\mathit{ind}}
%\newcommand{\prefix}{\mathit{prefix}}
\def\LRF{\mathit{lrf}}
%\newcommand{\distr}{\mathit{Distr}}
%\newcommand{\dirac}{\mathit{Dirac}}
\newcommand{\level}{\mathit{level}}
\newcommand{\period}{\mathit{period}}
\def\init{{\mathit{init}}}
\def\U{\until}
\def\PIMC{\textsl{MA}}
\def\Diamond{\pmb{\lozenge}}
\newcommand{\Suppbot}[1]{\boted{\mathrm{Supp}}(#1)}

\newcommand{\boted}[1]{#1_{\bot}}

% Family of ...
% \newcommand{\family}[2]{{{\{#1\}}_{#2}}}

% Automata and components
\newcommand{\pa}[1][P]{\aut[#1]}
\newcommand{\fps}[1][F]{\aut[#1]}
\newcommand{\dtmc}[1][D]{\aut[#1]}
\newcommand{\ctmc}[1][C]{\aut[#1]}
\newcommand{\ctmdp}[1][CM]{\aut[#1]}
\newcommand{\ctpa}[1][CP]{\aut[#1]}
\newcommand{\ma}[1][MA]{\aut[#1]}
\newcommand{\imc}[1][I]{\aut[#1]}
\newcommand{\internalActionSet}{\mathtt{H}}
\newcommand{\externalActionSet}{\mathtt{E}}
\newcommand{\initialDistribution}{\iota}
\newcommand{\transitionRelation}{\mathord{\rightarrow}}
\newcommand{\transitionProbability}{\mathbf{P}}
\newcommand{\transitionRate}{\mathbf{R}}
\newcommand{\paramSet}{\mathsf{P}}
%\newcommand{\algoTrue}{\ensuremath{\mathbf{true}}}
%\newcommand{\algoFalse}{\ensuremath{\mathbf{false}}}
%
%%\newcommand{\procedure}[1]{\textnormal{\scshape#1}}
%%\newcommand{\BREAKLOOP}{\STATE{\textbf{break};}}
%\newcommand{\SameProc}{\procedure{Same}}
%\newcommand{\MinimalProc}{\procedure{Minimal}}
%
%\newcommand{\SequenceOfFlowsProc}{\procedure{Smf}}
%\newcommand{\SequenceOfFlowsInitProc}{\procedure{Smf}_{\mathit{init}}}
%
%\newcommand{\StepCondition}{\procedure{StepCondition}}
\newcommand{\setcardinality}[1]{|#1|}


%\newcommand{\classToSplit}{{\mathcal C}}
%\newcommand{\splitAction}{a}
%\newcommand{\splitDistribution}{\gd}
%
%\newcommand{\listener}[1]{\mathit{Listener}(#1)}
%\newcommand{\match}{\mathit{match}}


%%%%%%%%%%%%%%     COMMENTS FOR ROBUST OPTIMIZATION %%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\uncertainLP}{{ULP}}
\newcommand{\uncertaintySet}{\mathcal{Z}}
%\newcommand{\vector}[1]{\text{\bf #1}}


%%%%%%%%%%%%%








==> Further files apart from main tex/use-comments.tex <==
\setboolean{useComments}{FALSE}

==> bibtex.tex <==
@inproceedings{DBLP:IG15,
	author = {Association, Information Resources},
	title = {Standard and Standardization: Concepts, Methodologies, Tools and Applications},
	publisher = {USA: IGI Global},
	year = {2015}
}
@phdthesis{Hashemi17,
	author    = {Vahid Hashemi},
	title     = {Decision algorithms for modelling, optimal control and verification
	of probabilistic systems},
	school    = {Saarland University, Saarbr{\"{u}}cken, Germany},
	year      = {2017},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{hashemi2016compositional,
	title={Compositional bisimulation minimization for interval Markov decision processes},
	author={Hashemi, Vahid and Hermanns, Holger and Song, Lei and Subramani, K and Turrini, Andrea and Wojciechowski, Piotr},
	booktitle={Language and Automata Theory and Applications},
	pages={114--126},
	year={2016},
	organization={Springer}
}
@inproceedings{GeblerHT12,
	author="Gebler, Daniel
	and Hashemi, Vahid
	and Turrini, Andrea",
	title="Computing Behavioral Relations for Probabilistic Concurrent Systems",
	booktitle= "ROCKS 2012",
	year="2014",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="117--155",
}
@inproceedings{DBLP:BC14,
	author = {Christiane Brünglinghaus},
	title = {Elektronik und Software beherrschen Innovationen im Auto},
	publisher = {Springer Professional},
	year = {2014}
}

@inproceedings{DBLP:conf/ecsa/HageHM20,
	author    = {Hassan Hage and
	Vahid Hashemi and
	Frank Mantwill},
	title     = {Towards a Systems Engineering Based Automotive Product Engineering
	Process},
	booktitle = {Software Architecture - 14th European Conference},
	series    = {Communications in Computer and Information Science},
	volume    = {1269},
	pages     = {527--541},
	publisher = {Springer},
	year      = {2020}
}
@inproceedings{DBLP:DuranRS18,
	author = {Francisco Duran and Camilo Rocha and Gwen Salaün},
	title = {Stochastic Analysis of BPMN with Time in Rewriting Logic},
	booktitle = {Science of Computer Programming}, 
	pages     = {168, pp. 1-17},
	publisher = {Elsevier},
	year = {2018}
}
@inproceedings{DBLP:LukeH14,
	author = {Luke Hebert},
	title = {Specification, Verification and Optimisation of Business Process},
	publisher = {Technical University of Denmark},
	year = {2014}
}
@book{bhise2017automotive,
	title={Automotive Product Development: A Systems Engineering Implementation},
	author={Bhise, V.D.},
	isbn={9781351645812},
	year={2017},
	publisher={CRC Press}
}
@book{verein2004entwicklungsmethodik,
	title={Entwicklungsmethodik f{\"u}r mechatronische Systeme VDI 2206: Design methodology for mechatronic systems},
	author={Verein Deutscher Ingenieure VDI},
	year={2004},
	publisher={VDI}
}
@book{weber2009automotive,
	title={Automotive Development Processes: Processes for Successful Customer Oriented Vehicle Development},
	author={Weber, J.},
	isbn={9783642012532},
	lccn={2009928427},
	year={2009},
	publisher={Springer Berlin Heidelberg}
}
@MISC{OMG:objectmanagementgroup,
	AUTHOR       = "OMG Object Management Group",
	TITLE        = "Business Process Model and Notation (BPMN)",
	YEAR         = "2014",
	HOWPUBLISHED = "Website",
	URL =      {https://www.omg.org/spec/BPMN};

}
@book{DBLP:journals/fac/HanssonJ94,
	author    = {Hans Hansson and
	Bengt Jonsson},
	title     = {A Logic for Reasoning about Time and Reliability},
	journal   = {Formal Asp. Comput.},
	volume    = {6},
	number    = {5},
	year      = {1994},
	pages     = {512-535},
	ee        = {http://dx.doi.org/10.1007/BF01211866},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}
@book{Aspice,
	title = {Automotive SPICE Process Assessment / Reference Model},
	author = {VDA QMC Working Group 13 / Automotive SIG},
	year = {2017},
	publisher = {Automotive SPICE},
	keywords = {Software}
}

@inproceedings{DaveP11,
	author = {Dave Parker},
	title = {Lecture 14 Model Checking for {MDP}s},
	publisher = {University of Oxford, Department Science},
	year = {2011}
}
@inproceedings{DBLP:conf/formats/AndovaHK03,
	author    = {Suzana Andova and
	Holger Hermanns and
	Joost{-}Pieter Katoen},
	editor    = {Kim Guldstrand Larsen and
	Peter Niebert},
	title     = {Discrete-Time Rewards Model-Checked},
	booktitle = {Formal Modeling and Analysis of Timed Systems: First International
	Workshop, {FORMATS} 2003, Marseille, France, September 6-7, 2003.
	Revised Papers},
	series    = {Lecture Notes in Computer Science},
	volume    = {2791},
	pages     = {88--104},
	publisher = {Springer},
	year      = {2003},
	
}
@InProceedings{CHH+13,
	author={Taolue Chen and Ernst Moritz Hahn and Tingting Han and Marta Kwiatkowska and Hongyang Qu and Lijun Zhang},
	title={Model Repair for {Markov} Decision Processes},
	booktitle={Proc. 7th International Symposium on Theoretical Aspects of Software Engineering (TASE'13)},
	year={2013},
	pages={85--92},
	publisher={IEEE},
}
@book{dajsuren2019automotive,
	title={Automotive Systems and Software Engineering: State of the Art and Future Trends},
	author={Dajsuren, Y. and van den Brand, M.},
	isbn={9783030121570},
	year={2019},
	publisher={Springer International Publishing}
}
@book{bhise2017automotive,
	title={Automotive Product Development: A Systems Engineering Implementation},
	author={Bhise, V.D.},
	isbn={9781351645812},
	year={2017},
	publisher={CRC Press}
}
@inproceedings{Gausemeier2013SEInDerIndustriellenPraxis,
	title={Systems Engineering in der industriellen Praxis},
	author={Jürgen Gausemeier and Roman Dumitrescu and Daniel Steffen and Anja Czaja and Olga Wiederkehr and Christian Tschirner},
	year={2013},
	publisher={Heinz Nixdorf Institut, Frauenhofer Institut, UNITY AG}
}
@inproceedings{Glinz2007,
	author = {Martin Glinz, Samuel Fricker},
	title = {Software Quality Selected Chapter, Chapter 7, Process quality},
	publisher = {University of Zürich, Institut for Informatics},
	year = {2007}
}

@InProceedings{10.1007/3-540-46002-0_5,
	author="Kwiatkowska, Marta
	and Norman, Gethin
	and Parker, David",
	editor="Katoen, Joost-Pieter
	and Stevens, Perdita",
	title="Probabilistic Symbolic Model Checking with PRISM: A Hybrid Approach",
	booktitle="Tools and Algorithms for the Construction and Analysis of Systems",
	year="2002",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="52--66",
	abstract="In this paper we introduce PRISM, a probabilistic model checker, and describe the efficient symbolic techniques we have developed during its implementation. PRISM is a tool for analysing probabilistic systems. It supports three models: discrete-time Markov chains, continuous-time Markov chains and Markov decision processes. Analysis is performed through model checking specifications in the probabilistic temporal logics PCTL and CSL. Motivated by the success of model checkers such as SMV, which use BDDs (binary decision diagrams), we have developed an implementation of PCTL and CSL model checking based on MTBDDs (multi-terminal BDDs) and BDDs. Existing work in this direction has been hindered by the generally poor performance of MTBDD-based numerical computation, which is often substantially slower than explicit methods using sparse matrices. We present a novel hybrid technique which combines aspects of symbolic and explicit approaches to overcome these performance problems. For typical examples, we achieve orders of magnitude speed-up compared to MTBDDs and are able to almost match the speed of sparse matrices whilst maintaining considerable space savings.",
	isbn="978-3-540-46002-2"
}

@inproceedings{krishna:hal-01591665,
	TITLE = {{VBPMN: Automated Verification of BPMN Processes}},
	AUTHOR = {Krishna, Ajay and Poizat, Pascal and Sala{\"u}n, Gwen},
	URL = {https://hal.inria.fr/hal-01591665},
	BOOKTITLE = {{13th International Conference on integrated Formal Methods (iFM 2017)}},
	ADDRESS = {Turin, Italy},
	YEAR = {2017},
	MONTH = Sep,
	KEYWORDS = {business processes ; BPMN ; verification ; evolution ; tool ; process algebra ; LNT ; labelled transition system ; model transformation},
	PDF = {https://hal.inria.fr/hal-01591665/file/main.pdf},
	HAL_ID = {hal-01591665},
	HAL_VERSION = {v1},
}


@article{DBLP:journals/ijseke/Lam10,
	author    = {Vitus S. W. Lam},
	title     = {Formal Analysis of {BPMN} Models: a NuSMV-Based Approach},
	journal   = {Int. J. Softw. Eng. Knowl. Eng.},
	volume    = {20},
	number    = {7},
	pages     = {987--1023},
	year      = {2010},
	url       = {https://doi.org/10.1142/S0218194010005079},
	timestamp = {Wed, 22 Jul 2020 22:06:17 +0200},
	biburl    = {https://dblp.org/rec/journals/ijseke/Lam10.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{doi:10.1080/00207540701199677,
	author = { C.   Ou-Yang  and  Y. D.   Lin },
	title = {{BPMN}-based business process model feasibility analysis: a {P}etri net approach},
	journal = {International Journal of Production Research},
	volume = {46},
	number = {14},
	pages = {3763-3781},
	year  = {2008},
	publisher = {Taylor and Francis},	
	URL = { 
	https://doi.org/10.1080/00207540701199677
	},
	
}

@article{article,
	author = {Mendoza Morales, Luis},
	year = {2014},
	month = {08},
	pages = {3-3},
	title = {Business Process Verification: The Application of Model Checking and Timed Automata},
	volume = {17},
	journal = {CLEI Electronic Journal},
}

@inproceedings{enterprisearchitect,
	TITLE = {{Enterprise Architect 15.2 [Software]}},
	AUTHOR = {Sparx Systems Central Europe},
	URL = {https://www.sparxsystems.de},
	YEAR = {2021},
}

@inproceedings{DBLP:DaclinVV15,
	author = {Nicolas Daclin and Bruno Vallespir and Capurlat Vincent},
	title = {Enabling model checking for collaborative process analysis: from BPMN to ‘Network of Timed Automata’},
	publisher = {Taylor and Francis},
	booktitle = {Enterprise Inforation Systems}, 
	volume = {9},
	pages     = {279--299},
	year = {2015}
}

@Inbook{Valmari1998,
	author={Valmari, Antti},
	editor={Reisig, Wolfgang
	and Rozenberg, Grzegorz},
	title={The state explosion problem},
	bookTitle={Lectures on Petri Nets I: Basic Models: Advances in Petri Nets},
	year={1998},
	publisher={Springer Berlin Heidelberg},
	address={Berlin, Heidelberg},
	pages={429--528},
}

@inproceedings{HahnHWZ10,
	author    = {Ernst Moritz Hahn and
	Holger Hermanns and
	Bj{\"o}rn Wachter and
	Lijun Zhang},
	title     = {PARAM: A Model Checker for Parametric Markov Models},
	booktitle = {CAV},
	year      = {2010},
	pages     = {660-664},
}
@article{DBLP:journals/corr/DehnertJK016,
	author    = {Christian Dehnert and
	Sebastian Junges and
	Joost{-}Pieter Katoen and
	Matthias Volk},
	title     = {The Probabilistic Model Checker Storm (Extended Abstract)},
	journal   = {CoRR},
	volume    = {abs/1610.08713},
	year      = {2016},
	url       = {http://arxiv.org/abs/1610.08713},
	eprinttype = {arXiv},
	eprint    = {1610.08713},
	timestamp = {Mon, 13 Aug 2018 16:48:38 +0200},
	biburl    = {https://dblp.org/rec/journals/corr/DehnertJK016.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{hartmanns2014modest,
	title={The Modest Toolset: An integrated environment for quantitative modelling and verification},
	author={Hartmanns, Arnd and Hermanns, Holger},
	booktitle={International Conference on Tools and Algorithms for the Construction and Analysis of Systems},
	pages={593--598},
	year={2014},
	organization={Springer}
}

@inproceedings{hahn2014iscas,
	title={iscas M c: a web-based probabilistic model checker},
	author={Hahn, Ernst Moritz and Li, Yi and Schewe, Sven and Turrini, Andrea and Zhang, Lijun},
	booktitle={International Symposium on Formal Methods},
	pages={312--317},
	year={2014},
	organization={Springer}
}

@Inproceedings{10.1007/978-3-319-43425-4_4,
	author="Hahn, Ernst Moritz
	and Hashemi, Vahid
	and Hermanns, Holger
	and Turrini, Andrea",
	editor="Agha, Gul
	and Van Houdt, Benny",
	title="Exploiting Robust Optimization for Interval Probabilistic Bisimulation",
	booktitle="Quantitative Evaluation of Systems",
	year="2016",
	publisher="Springer International Publishing",
	address="Cham",
	pages="55--71"
}
